RoboKeyGen: Robot Pose and Joint Angles Estimation via Diffusion-based 3D Keypoint Generation

Estimating robot pose and joint angles is significant in advanced robotics, enabling applications like robot collaboration and online hand-eye calibration.However, the introduction of unknown joint angles makes prediction more complex than simple robot pose estimation, due to its higher dimensionality.Previous methods either regress 3D keypoints directly or utilise a render&compare strategy. These approaches often falter in terms of performance or efficiency and grapple with the cross-camera gap problem.This paper presents a novel framework that bifurcates the high-dimensional prediction task into two manageable subtasks: 2D keypoints detection and lifting 2D keypoints to 3D. This separation promises enhanced performance without sacrificing the efficiency innate to keypoint-based techniques.A vital component of our method is the lifting of 2D keypoints to 3D keypoints. Common deterministic regression methods may falter when faced with uncertainties from 2D detection errors or self-occlusions.Leveraging the robust modeling potential of diffusion models, we reframe this issue as a conditional 3D keypoints generation task. To bolster cross-camera adaptability, we introduce theNormalised Camera Coordinate Space (NCCS), ensuring alignment of estimated 2D keypoints across varying camera intrinsics.Experimental results demonstrate that the proposed method outperforms the state-of-the-art render\&compare method and achieves higher inference speed.Furthermore, the tests accentuate our method's robust cross-camera generalisation capabilities.We intend to release both the dataset and code in https://nimolty.github.io/Robokeygen/

==> tables/angles.tex <==
\begin{tabular}{cccccc}
\toprule
Method      & $2.5^\circ$ & $5.0^\circ$ & $7.5^\circ$ & $10.0^\circ$ & $12.5^\circ$ \\ \midrule \midrule
                     & \multicolumn{5}{c}{RealSnense}                        \\ \midrule
Robopose\cite{Labbe2021SingleviewRP}             & 28.32     & 44.21     & 53.01     & 58.90      & 63.50     \\
Ours  & 37.48     & 59.79     & 71.60     & 78.21      & 82.32      \\ \midrule
                     & \multicolumn{5}{c}{Azure-Kinect}                      \\ \midrule 
Robopose\cite{Labbe2021SingleviewRP}              & 24.58     & 40.72     & 49.51     & 55.40      & 59.37      \\
Ours  & 28.68     & 46.25     & 56.37     & 62.64      & 67.54     \\ \bottomrule
\end{tabular}


==> tables/dream_tests.tex <==
\begin{tabular}{cccc}
\toprule
Method               &       AUC@0.1m & Median(m) & Mean(m) \\ \midrule \midrule
               \multicolumn{4}{c}{Panda 3CAM-RS\cite{Lee2019CameratoRobotPE}}             \\ \midrule
Robopose\cite{Labbe2021SingleviewRP} & 74.07   &    0.021    &  \textbf{0.029}   \\
Ours  &  \textbf{78.39} &   \textbf{0.018}    &   \textbf{0.029}  \\ \midrule
               \multicolumn{4}{c}{Panda 3CAM-AK\cite{Lee2019CameratoRobotPE}}             \\ \midrule
Robopose\cite{Labbe2021SingleviewRP} &  69.71  &    \textbf{0.021}    &   0.039  \\
Ours  & \textbf{69.86}  &    \textbf{0.021}    &   \textbf{0.036}  \\ \midrule
                \multicolumn{4}{c}{Panda ORB\cite{Lee2019CameratoRobotPE}}         \\ \midrule
Robopose\cite{Labbe2021SingleviewRP} & 60.70   &    0.031    &   0.043  \\
    Ours  &  \textbf{64.01}  &    \textbf{0.027}    &   \textbf{0.042}  \\ \bottomrule
\end{tabular}

==> tables/image_generation.tex <==
% \begin{tabular}{c|ccc}
% \toprule
% Method               & AUC@(60/100mm) & Median (mm) & Mean(mm) \\ \midrule \midrule
%                      & \multicolumn{3}{c}{Ours-RS}             \\ \midrule 
% Image Generation     & 0.59 / 4.50    & 130.96      & 158.70   \\
% Ours  & 56.46 / 72.93  & 21.60       & 28.45    \\ \midrule
% \multicolumn{1}{l}{} & \multicolumn{3}{c}{Ours-Kinect}         \\ \midrule
% Image Generation     & 0.00 / 0.00    & 400.89      & 403.72   \\
% Ours  & 45.76 / 63.33  & 27.75       & 44.55   \\ \bottomrule
% \end{tabular}

\begin{tabular}{cccc}
\toprule
Method               & AUC@0.1m & Median(m) & Mean(m) \\ \midrule \midrule
                     \multicolumn{4}{c}{RealSense-Franka}             \\ \midrule 
Image Generation     & 4.50    & 0.131      & 0.159   \\
Ours  & 72.93  & 0.022       & 0.028    \\ \midrule
                     \multicolumn{4}{c}{AzureKinect-Franka}         \\ \midrule
Image Generation     & 0.00    & 0.401      & 0.404   \\
Ours  & 63.33  & 0.028       & 0.045   \\ \bottomrule
\end{tabular}

==> tables/main_results_010.tex <==
\begin{tabular}{c|c|ccc|ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Joint angles} & \multicolumn{3}{c}{Ours-RS} & \multicolumn{3}{c}{Ours-Kinect} \\ \cmidrule{3-8}
 & & AUC@100mm$\uparrow$ & Median (mm)$\downarrow$ & Mean (mm)$\downarrow$ & AUC@100mm$\uparrow$ & Median (mm)$\downarrow$ & Mean (mm)$\downarrow$ \\ \midrule \midrule
RoboPose & \multirow{4}{*}{\ding{55}}       & 31.78          & 72.67           & 105.32          & 39.83          & 47.3           & 82.93            \\ 
SPDH-HRNet              &                   & 3.39            & 1366.18         & 1297.10         & 0.00            & 643.35          & 668.79            \\ 
SPDH-SH                 &                   & 17.24            & 251.17          & 271.85          & 0.00            & 844.09          & 853.98            \\ 
% SPDH-RESNET(Ours)       &                   & 46.09           & 49.33           & 55.66           & 0.00            & 655.09          & 676.79            \\ 
% SPDH-HRNet-Reprojected  &                   & 40.67           & 30.15           & 61.45           & 11.11           & 90.70           & 132.06            \\ 
% SPDH-SH-Reprojected     &                   & 28.54           & 38.91           & 121.87          & 13.87           & 74.73           & 153.20            \\ 
% SPDH-RESNET-Reprojected                   & 46.34           & 28.98           & 34.09           & 0.2             & 126.12          & 184.28            \\ 
Ours Tracking (ddim)    &                   & \textbf{72.93}  & \textbf{21.60}  & \textbf{28.45}  & \textbf{63.33}  & \textbf{27.75}  & \textbf{44.55}    \\ \midrule
Dream-VGG-Q & \multirow{8}{*}{\checkmark}   & 32.35           & 75.29           & 352.28          & 27.48           & 80.23          & 244.39             \\
Dream-VGG-F             &                   & 2.31            & 1384.69          & /               & 0.37               & 1471.00          & /                 \\
Dream-RESNET-H          &                   &            &            &            &            &           &             \\
Dream-RESNET-F          &                   & 38.6           & 53.44           & /               & 20.31           & 1095.48          & /                 \\
RoboPose                &                   & 44.18          & 49.77           & 61.52           & 41.59           & 52.93           & 61.62             \\
SGTAPose               &                   &     52.70       &    37.06        &    24.29       &      39.97      &    58.59        &        93.80       \\
CtRNet                  &                   &                 &                 &                 &                 &                 &                   \\
Ours Tracking (ddim)    &                   & \textbf{74.76}  & \textbf{19.91}  & \textbf{26.48}  & \textbf{66.84}  & \textbf{24.52}  & \textbf{40.70}    \\ \bottomrule
\end{tabular}

==> tables/nco_space_010.tex <==
\begin{tabular}{ccccccc}
Method                             & \multicolumn{3}{c}{Ours-RS}       & \multicolumn{3}{c}{Ours-Kinect}     \\
                                   & AUC@100mm & Median (mm) & Mean(mm) & AUC (100mm) & Median (mm) & Mean(mm) \\
Ours w/o NCO (gt 2D)               & 24.98     & 75.62       & 75.79    & 0.00       & 695.64     & 707.38   \\
Ours w/o NCO Tracking (ddim gt 2D) & 9.33     & 95.10      & 97.56    & 0.00       & 768.64      & 800.55   \\
Ours w/o NCO                       & 0.00     & 422.93      & 433.85   & 0.00       & 379.47      & 405.45   \\
Ours w/o NCO Tracking (ddim)       & 0.00     & 412.11      & 432.87  & 0.00       & 396.25      & 409.62   \\
Ours Tracking (ddim)               & 72.93    & 21.60       & 28.45    & 63.33      & 25.75       & 44.55   
\end{tabular}


==> tables/num_samples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{tabular}{c|c|ccc|ccc}
% \toprule
% \multirow{2}{*}{Method}     & \multirow{2}{*}{Joint angles}      & \multicolumn{3}{c}{Ours-RS}       & \multicolumn{3}{c}{Ours-Kinect}        \\ \cmidrule{3-8} &  & AUC@(60/100mm)  $\uparrow$    & Median (mm)  $\downarrow$ & Mean(mm) $\downarrow$ & AUC@(60/100mm) $\uparrow$   & Median (mm) $\downarrow$ & Mean(mm) $\downarrow$ \\ \midrule \midrule

% %\multirow{2}{*}{Method} & \multirow{2}{*}{Joint angles} & \multicolumn{4}{c}{Ours-RS} & \multicolumn{4}{c}{Ours-Kinect} \\ \cmidrule{3-10} &
% % & AUC@100mm$\uparrow$ & AUC@60mm$\uparrow$ & Median (mm)$\downarrow$ & Mean (mm)$\downarrow$ & AUC@100mm$\uparrow$ & AUC@60mm$\uparrow$ & Median (mm)$\downarrow$ & Mean (mm)$\downarrow$ \\ \midrule \midrule

                     
% Ours Tracking (s=1)  & \multirow{6}{*}{\ding{55}} & 41.67 / 61.92 & 32.08       & 39.84    & 37.68 / 57.57 & 34.16       & 50.87    \\
% Ours Tracking (s=2)  &                   & 48.51 / 67.34 & 26.73       & 34.11    & 41.73 / 60.55 & 31.15       & 47.61    \\
% Ours Tracking (s=5)  &                   & 54.10 / 71.31 & 23.23       & 30.08    & 44.51 / 62.48 & 28.79       & 45.64    \\
% Ours Tracking (s=10) &                   & 56.47 / 72.93 & 21.60       & 28.45    & 45.76 / 63.33 & 27.75       & 44.55    \\
% Ours Tracking (s=15) &                   & 57.01 / 73.27 & 21.45       & 28.11    & 45.98 / 63.47 & 27.55       & 44.53    \\
% Ours Tracking (s=20) &                   & 57.35 / 73.50 & 21.03       & 27.99    & 46.13 / 63.59 & 27.58       & 44.38    \\ \midrule
% Ours Tracking (s=1)  & \multirow{6}{*}{\checkmark} & 44.59 / 63.91 & 30.21       & 47.10    & 42.38 / 60.97 & 30.83       & 47.10    \\
% Ours Tracking (s=2)  &                   & 51.58 / 69.38 & 24.60       & 31.92    & 46.32 / 63.82 & 28.22       & 43.87    \\
% Ours Tracking (s=5)  &                   & 57.11 / 73.24 & 21.45       & 28.01    & 49.56 / 66.00 & 25.51       & 41.51    \\
% Ours Tracking (s=10) &                   & 59.34 / 74.76 & 19.91       & 26.48    & 50.82 / 66.84 & 24.52       & 40.70    \\
% Ours Tracking (s=15) &                   & 59.82 / 75.07 & 19.72       & 26.15    & 51.02 / 66.97 & 24.49       & 40.59    \\
% Ours Tracking (s=20) &                   & 60.13 / 75.28 & 19.34       & 25.94    & 51.19 / 67.09 & 24.49       & 40.47   \\ \bottomrule
% \end{tabular}

\begin{tabular}{l|ccc}
\toprule
Method               &       AUC@0.1m & Median(m) & Mean(m) \\ \midrule \midrule
               & \multicolumn{3}{c}{RealSense}             \\ \midrule
Ours ($K=1$) &  61.92  &    0.033    &   0.040  \\
Ours ($K=2$) &  67.34  &   0.027     &  0.034   \\
Ours ($K=5$) &  71.31  &     0.023   &   0.031  \\
Ours ($K=10$)&  72.93  &    0.022    &   0.028  \\ 
% Ours (s=15) &  73.27  &   0.021     &   0.028  \\
% Ours (s=20) &  73.27  &     0.021   &  0.028   \\
Ours ($K=30$) &  73.73  &   0.021     &  0.028   \\
Ours ($K=50$) &  73.95  &    0.021    &   0.027  \\
Ours ($K=80$) &  74.11  &    0.021    &   0.027  \\
Ours ($K=100$) &  74.11  &     0.021   &   0.027  \\ \midrule
                     &  \multicolumn{3}{c}{Azure-Kinect}         \\ \midrule
Ours ($K=1$) & 57.57   &    0.034    &  0.051   \\
Ours ($K=2$) &  60.55   &     0.031   &  0.048   \\
Ours ($K=5$) &  62.48  &    0.029    &   0.046  \\
Ours ($K=10$)&   63.33 &   0.028     &  0.045   \\ 
% Ours (s=15) &  63.47  &   0.028     &   0.045  \\
% Ours (s=20) &  63.59  &    0.028    &   0.044  \\
Ours ($K=30$) &  63.67  &   0.028     &  0.044   \\
Ours ($K=50$) &  63.83  &    0.027   &   0.044  \\
Ours ($K=80$) &  63.84  &     0.027   &   0.044  \\
Ours ($K=100$) &  63.84  &    0.027    &   0.044  \\ \bottomrule
\end{tabular}


